Non-degenerate bilinear forms in characteristic 2, related contact forms, simple Lie algebras and superalgebras

Non-degenerate bilinear forms over fields of characteristic 2, in particular, non-symmetric ones, are classified with respect to various equivalences, and the Lie algebras preserving them are described. Although it is known that there are two series of distinct finite simple Chevalley groups preserving the non-degenerate symmetric bilinear forms on the space of even dimension, the description of simple Lie algebras related to the ones that preserve these forms is new. The classification of 1-forms is shown to be related to one of the considered equivalences of bilinear forms. A version of the above results for superspaces is also given.

==> DAL-defs.tex <==
\usepackage{amsmath}
\usepackage{amssymb}

\newcommand {\noqed}
 {\renewcommand {\qed} {}}

\usepackage{bbm}
\newcommand{\One}{\mathbbmss{1}}

% ===========================================
%
%                New Symbols
%
% ===========================================
\newcommand {\supplus}{\mathop{{\supset}\llap{\raise
0.5pt\hbox{\normalfont\small+}\hskip 0.5pt}}}
%semidirect sum, the ideal on the left

\newcommand {\subplus}{\mathop{{\subset}\llap{\raise
0.5pt\hbox{\normalfont\small+}\hskip 0.5pt}}}
%semidirect sum, the ideal on the right

\newcommand {\divby}  {\lower 0.15ex \hbox{\,\vdots\,}}
%
% ===========================================

\newcommand {\Aee}    {{\mathbb  A}}
\newcommand {\Cee}    {{\mathbb  C}}
\newcommand {\Eee}    {{\mathbb  E}}
\newcommand {\Fee}    {{\mathbb  F}}
\newcommand {\Gee}    {{\mathbb  G}}
\newcommand {\Hee}    {{\mathbb  H}}
\newcommand {\Kee}    {{\mathbb  K}}
\newcommand {\Nee}    {{\mathbb  N}}
\newcommand {\Oee}    {{\mathbb  O}}
\newcommand {\Pee}    {{\mathbb  P}}
\newcommand {\Qee}    {{\mathbb  Q}}
\newcommand {\Ree}    {{\mathbb  R}}
\newcommand {\Tee}    {{\mathbb T}}
\newcommand {\Uee}    {{\mathbb  U}}
\newcommand {\Zee}    {{\mathbb  Z}}

\newcommand {\fa}     {{\mathfrak{a}}}
\newcommand {\fA}     {{\mathfrak{A}}}
\newcommand {\fab}    {{\mathfrak{ab}}}
\newcommand {\fag}    {{\mathfrak{ag}}}
\newcommand {\fas}    {{\mathfrak{as}}}
\newcommand {\faut}   {{\mathfrak{aut}}}
\newcommand {\fb}     {{\mathfrak{b}}}
\newcommand {\fc}    {{\mathfrak{c}}}
\newcommand {\fcg}    {{\mathfrak{cg}}}
\newcommand {\fcsvect} {{\mathfrak{csvect}}}
\newcommand {\fcvect}   {{\mathfrak{cvect}}}
\newcommand {\fD}     {{\mathfrak{D}}}   %
\newcommand {\fder}   {{\mathfrak{der}}}   %
\newcommand {\fdiff}  {{\mathfrak{diff}}}
\newcommand {\fdg}    {{\mathfrak{dg}}}
\newcommand {\fd}     {{\mathfrak{d}}}
\newcommand {\fe}     {{\mathfrak{e}}}
\newcommand {\feg}    {{\mathfrak{eg}}}
\newcommand {\ff}     {{\mathfrak{f}}}
\newcommand {\fF}     {{\mathfrak{F}}}
\newcommand {\fg}     {{\mathfrak{g}}}    %
\newcommand {\fG}     {{\mathfrak{G}}}    %
\newcommand {\fgl}    {{\mathfrak{gl}}}  %
\newcommand {\fGL}    {{\mathfrak{GL}}}  %
\newcommand {\fh}     {{\mathfrak{h}}}
\newcommand {\fhei}   {{\mathfrak{hei}}}
\newcommand {\fii}    {{\mathfrak{i}}}    %
\newcommand {\fI}    {{\mathfrak{I}}}    %
\newcommand {\fk}     {{\mathfrak{k}}}
\newcommand {\fkas}     {{\mathfrak{kas}}}
\newcommand {\fl}     {{\mathfrak{l}}}
\newcommand {\fL}     {{\mathfrak{L}}}
\newcommand {\fle}    {{\mathfrak{le}}}
\newcommand {\fM}     {{\mathfrak{M}}}   %
\newcommand {\fm}     {{\mathfrak{m}}}
\newcommand {\fN}     {{\mathfrak{N}}}  %
\newcommand {\fn}     {{\mathfrak{n}}}
\newcommand {\fns}     {{\mathfrak{ns}}}
\newcommand {\fo}     {{\mathfrak{o}}}
\newcommand {\fosp}   {{\mathfrak{osp}}}
\newcommand {\fp}    {{\mathfrak{p}}}   %
\newcommand {\fpe}    {{\mathfrak{pe}}}   %
\newcommand {\fpg}    {{\mathfrak{pg}}}
\newcommand {\fpm}    {{\mathfrak{pm}}}
\newcommand {\fpgl}   {{\mathfrak{pgl}}}
\newcommand {\fpo}    {{\mathfrak{po}}}
\newcommand {\fPo}    {{\mathfrak{Po}}}
\newcommand {\fpsl}   {{\mathfrak{psl}}}
\newcommand {\fpq}    {{\mathfrak{pq}}}
\newcommand {\fpsh}   {{\mathfrak{psh}}}
\newcommand {\fpsq}   {{\mathfrak{psq}}}
\newcommand {\fq}     {{\mathfrak{q}}}
\newcommand {\fr}     {{\mathfrak{r}}}
\newcommand {\fqdiff} {{\mathfrak{qdiff}}}
\newcommand {\fs}     {{\mathfrak{s}}}
\newcommand {\fsa}    {{\mathfrak{sa}}}
\newcommand {\fsb}    {{\mathfrak{sb}}}
\newcommand {\fsg}    {{\mathfrak{sg}}}
\newcommand {\fsh}    {{\mathfrak{sh}}}
\newcommand {\fsi}    {{\mathfrak{si}}}
\newcommand {\fsl}    {{\mathfrak{sl}}}
\newcommand {\fsle}   {{\mathfrak{sle}}}
\newcommand {\fsm}    {{\mathfrak{sm}}}
\newcommand {\fsp}    {{\mathfrak{sp}}}
\newcommand {\fspe}   {{\mathfrak{spe}}}
\newcommand {\fspo}   {{\mathfrak{spo}}}
\newcommand {\fsq}    {{\mathfrak{sq}}}
\newcommand {\fss}    {{\mathfrak{ss}}}
\newcommand {\fst}    {{\mathfrak{st}}}
\newcommand {\fsvect} {{\mathfrak{svect}}}
\newcommand {\fsu}    {{\mathfrak{su}}}
\newcommand {\ft}     {{\mathfrak{t}}}
\newcommand {\fu}     {{\mathfrak{u}}}
\newcommand {\fv}     {{\mathfrak{v}}}     %
\newcommand {\fvas}     {{\mathfrak{vas}}}     %
\newcommand {\fvle}     {{\mathfrak{vle}}}     %
\newcommand {\fvect}  {{\mathfrak{vect}}}   %
\newcommand {\fvir}   {{\mathfrak{vir}}}
\newcommand {\fw}     {{\mathfrak{w}}}
\newcommand {\fwitt}  {{\mathfrak{witt}}}
\newcommand {\fx}  {{\mathfrak{x}}}
\newcommand {\fz}     {{\mathfrak{z}}}
\newcommand {\fZ}     {{\mathfrak{Z}}}

\newcommand {\cal} {\mathcal}

\newcommand {\cA}     {{\cal A}}
\newcommand {\cB}     {{\cal B}}
\newcommand {\cC}     {{\cal C}}
\newcommand {\cD}     {{\cal D}}
\newcommand {\cE}     {{\cal E}}
\newcommand {\cF}     {{\cal F}}
\newcommand {\cG}     {{\cal G}}
\newcommand {\cH}     {{\cal H}}
\newcommand {\cI}     {{\cal I}}
\newcommand {\cJ}     {{\cal J}}
\newcommand {\cK}     {{\cal K}}
\newcommand {\cL}     {{\cal L}}
\newcommand {\cM}     {{\cal M}}
\newcommand {\cN}     {{\cal N}}
\newcommand {\cO}     {{\cal O}}
\newcommand {\cP}     {{\cal P}}
\newcommand {\cR}     {{\cal R}}
\newcommand {\cS}     {{\cal S}}
\newcommand {\cT}     {{\cal T}}
\newcommand {\cU}     {{\cal U}}
\newcommand {\cV}     {{\cal V}}
\newcommand {\cW}     {{\cal W}}
\newcommand {\cX}     {{\cal X}}
\newcommand {\cZ}     {{\cal Z}}

% ===========================================
%
%                Operators
%
% ===========================================

\def \opname#1#2%
  {\expandafter\newcommand \csname #1\endcsname {{\mathop{#2}\nolimits}}}

%\def\rmname#1%
%  {\expandafter\newcommand \csname #1\endcsname
%     {{\mathop{\text{\normalshape\rm #1}}\nolimits}}}

\newcommand{\rmname}[1]
  {\expandafter\newcommand \csname #1\endcsname {{\operatorname{#1}}}}

\newcommand{\rmnameii}[2]
  {\expandafter\newcommand \csname #1\endcsname {{\operatorname{#2}}}}

\newcommand{\bra}[1] {\langle #1 |}
\newcommand{\ket}[1] {| #1 \rangle}

\rmname{act} \rmname{Ad} \rmname{Add} \rmname{ad} \rmname{Alt}
\rmname{alt} \rmname{Ann} \rmname{antidiag} \rmname{Ber}
\rmname{ber} \rmname{Bil} \rmname{Br} \rmname{card} \rmname{ch}
\rmname{Char} \rmname{cem} \rmname{cj} \rmname{Cliff}
\rmname{cntr} \rmname{codim} \rmname{coind} \rmname{const}
\rmname{col} \rmname{cork} \rmname{cpr} \rmname{diag}
 \rmnameii{Div}{div} \rmname{Def} \rmname{Deg}
\rmname{Der} \rmname{Diff} \rmname{Dim} \rmname{End} \rmname{Even}
\rmname{Ext} \rmname{gr} \rmname{Hom} \rmname{HT}
\rmnameii{Ht}{ht} \rmname{hwt} \rmname{Id} \rmname{id}
\rmname{ind} \rmname{Ind} \rmname{Inf} \rmname{irr} \rmname{Le}
\rmname{Lie} \rmname{lwt} \rmname{mult} \rmname{Mat} \rmname{Mor}
\rmname{nm} \rmname{Ob} \rmname{Odd} \rmname{Osc} \rmname{per}
\rmname{Pic} \rmname{pr} \rmname{pro} \rmname{Prime} \rmname{Proj}
\rmname{prt} \rmname{pt} \rmname{Q} \rmname{qet} \rmname{qtr}
\rmname{rd} \rmname{rk} \rmname{row} \rmname{Res} \rmname{salt}
\rmname{Sch} \rmname{SBr} \rmname{sdim}\rmname{scalar}
\rmname{Ser} \rmname{sign} \rmname{Smbl} \rmname{spin}
\rmname{ssym} \rmname{str} %\rmname{st}
\rmname{sgn} \rmname{sq}
\rmname{symm} \rmname{supp} \rmname{Supp} \rmname{St}
\rmname{Spec} \rmname{Spm} \rmname{tr} \rmname{vpt} \rmname{Vect}
\rmname{weyl} \rmname{Weyl} \rmname{Witt}

\opname{vvol}  {{v\hspace{-0.1ex}o\hspace{-0.02ex}l\/}}
\opname{pnt}  {\text{\normalfont pt}} \opname{Span} {{Span}}
\opname{slim} {\overline{\lim}} \opname{Vol}
{{V\hspace{-0.55ex}o\hspace{-0.02ex}l\/}} \opname{Par}
{{P\hspace{-0.3ex}a\hspace{-0.05ex}r\/}}

% ===========================================
%
%      Abbreviations
%
% ===========================================

\newcommand {\ev} {{\bar0}}
\newcommand {\od} {{\bar1}}
\newcommand {\eps} {\varepsilon}
\newcommand {\degree}  {{}^\circ}
\newcommand {\tto} {\longrightarrow}
\newcommand {\pder}[1] {{\frac{\partial}{\partial {#1}}}}
\newcommand {\pderf}[2] {{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand {\pders}[1] {{\partial/\partial {#1}}}
\newcommand {\pderfs}[2] {{\partial {#1}/\partial {#2}}}


% ===========================================
%
%     Bold dots
%
% ===========================================

\newcommand {\bdot} [1] {{\bf{\dot{\mit #1}}}}    % bold \dot
\newcommand {\bddot}[1] {{\bf{\ddot{\mit #1}}}}   % bold \ddot
\newcommand {\bcdot}   {\mathbin{\hbox{\raise.4ex\hbox{\bf.}}}} % bold \cdot


\newcommand {\secno} {}
\newcommand {\ssecfont} {\normalfont\bf}
\newcommand {\secfont} {\large\bf}

\ifsmart

\makeatletter

\theoremstyle{plain}
\@@newtheorem*{Theorem}{\secno Theorem}
\@@newtheorem*{Lemma}{\secno Lemma}
\@@newtheorem*{Proposition}{\secno Proposition}
\@@newtheorem*{Corollary}{\secno Corollary}
\@@newtheorem*{Statement}{\secno Statement}
\@@newtheorem*{Problem}{\secno Problem}
\@@newtheorem*{Question}{\secno Question}
\@@newtheorem*{Conjecture}{\secno Conjecture}

\theoremstyle{definition}
\@@newtheorem*{Example}{\secno Example}
\@@newtheorem*{Examples}{\secno Examples}
\@@newtheorem*{Convention}{\secno Convention}
\@@newtheorem*{Comment}{\secno Comment}

\theoremstyle{remark}

\@@newtheorem*{Remark}{\secno Remark}
\@@newtheorem*{Remarks}{\secno Remarks}
\@@newtheorem*{Exercise}{\secno Exercise}
\@@newtheorem*{Solution}{\secno Solution}
\@@newtheorem*{Hint}{\secno Hint}

\makeatother

\else

\newtheorem*{Theorem}{\secno Theorem}
\def \theTheorem {}
\newtheorem*{Lemma}{\secno Lemma}
\newtheorem*{Proposition}{\secno Proposition}
\newtheorem*{Corollary}{\secno Corollary}
\newtheorem*{Statement}{\secno Statement}
\newtheorem*{Problem}{\secno Problem}
\newtheorem*{Question}{\secno Question}
\newtheorem*{Conjecture}{\secno Conjecture}
\newenvironment {th*}[1]
    {\gdef\thname{#1} \begin{thn}}%
    {\end{thn}}
\newtheorem*{thn} {\thname}

\theoremstyle{definition}
\newtheorem*{Example}{\secno Example}
\newtheorem*{Examples}{\secno Examples}
\newtheorem*{Convention}{\secno Convention}
\newtheorem*{Comment}{\secno Comment}
\newtheorem*{Remark}{\secno Remark}

\newenvironment {ex*}[1]
    {\gdef\thname{#1} \begin{exn}}%
    {\end{exn}}
\newtheorem*{exn}{\thname}

\theoremstyle{remark}

%\newtheorem*{Remark}{\secno Remark}
\newtheorem*{Remarks}{\secno Remarks}
\newtheorem*{Exercise}{\secno Exercise}
\newtheorem*{Solution}{\secno Solution}
\newtheorem*{Hint}{\secno Hint}
\newenvironment {rem*}[1]
    {\gdef\thname{#1} \begin{remn}}%
    {\end{remn}}
\newtheorem*{remn}{\thname}

\fi

\makeatletter
\def\@secnumfont{\bfseries}
\def\section{\@startsection{section}{1}%
  \z@{.7\linespacing\@plus\linespacing}{.5\linespacing}%
  {\secfont\centering}}
\makeatother

\let\ssec\subsection


\newcommand {\ssbegin}[1]
  {\refstepcounter{subsection}
  \def \secno {\gdef \secno {}{\ssecfont \thesubsection.\hskip 2ex}%
  }%
   \begin{#1}}

\setcounter{tocdepth}{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pdr}[1]{\partial_{#1}}
\newcommand{\vf}{\varphi}


\newcommand{\ot}{\otimes}

